Where does In-context Translation Happen in Large Language Models

Self-supervised large language models have demonstrated the ability to perform Machine Translation (MT) via in-context learning, but little is known about where the model performs the task with respect to prompt instructions and demonstration examples. In this work, we attempt to characterize the region where large language models transition from in-context learners to translation models. Through a series of layer-wise context-masking experiments on \textsc{GPTNeo2.7B}, \textsc{Bloom3B}, \textsc{Llama7b} and \textsc{Llama7b-chat}, we demonstrate evidence of a "task recognition" point where the translation task is encoded into the input representations and attention to context is no longer necessary. We further observe correspondence between the low performance when masking out entire layers, and the task recognition layers. Taking advantage of this redundancy results in 45\% computational savings when prompting with 5 examples, and task recognition achieved at layer 14 / 32. Our layer-wise fine-tuning experiments indicate that the most effective layers for MT fine-tuning are the layers critical to task recognition.

==> tables/archive/masking_context_layers_description.tex <==

\begin{table*}[t]
\centering
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{l|c|c|l}

Name  & \texttt{Instr}   & \texttt{Ex}       &  \\
\toprule
%$\texttt{Instr}^{-} \texttt{Ex}^{-}$  & N & N & En: $\cdots$ Fr: \\

%$\texttt{Instr}^{-} \texttt{Ex}^{\bullet}$ 
\textcolor{blue}{$\overline{\texttt{Ex}}^{Mask}$} & N & \hl{Y} & \makecell[l]{\hl{En: $\cdots$ Fr: $\cdots$} En: $\cdots$ Fr:} \\
% \midrule
% $\texttt{Instr}^{\bullet}\texttt{Ex}^{-}$ &  \hl{Y} & N & \makecell[l]{\hl{Translate En to Fr:} En: $\cdots$ Fr:} \\

\midrule
%$\texttt{Instr}^{\circ} \texttt{Ex}^{\bullet}$ &  Y  & \hl{Y} & \makecell[l]{Translate En to Fr: \\ \hl{En: $\cdots$ Fr:$\cdots$} En: $\cdots$ Fr:}\\
%$\texttt{Instr}^{\circ} \texttt{Ex}^{\bullet}$, 
\textcolor{blue}{$\texttt{Instr},\overline{\texttt{Ex}}^{Mask}$} &  Y  & \hl{Y} & Translate En to Fr: \hl{En: $\cdots$ Fr:$\cdots$} En: $\cdots$ Fr:\\

\midrule
%$\texttt{Instr}^{\bullet} \texttt{Ex}^{\bullet}$ &  \hl{Y} & \hl{Y} & \makecell[l]{\hl{Translate En to Fr:} \\ \hl{En: $\cdots$ Fr:$\cdots$} En: $\cdots$ Fr:} \\
%$\texttt{Instr}^{\bullet} \texttt{Ex}^{\bullet}$, 
\textcolor{blue}{$\overline{\texttt{Instr}, \texttt{Ex}}^{Mask}$}  &  \hl{Y} & \hl{Y} & \hl{Translate En to Fr:} \hl{En: $\cdots$ Fr:$\cdots$} En: $\cdots$ Fr: \\

\end{tabular}}
\caption{For the prompt contexts of Instructions (\texttt{Instr}) and Examples ($\texttt{Ex}$). \newtext{The overline corresponds to the yellow highlights. This refers to attention masking from future time steps to previous time steps in the causal language models. $N$ and $Y$ refer to absence and presence of either Instruction of Examples. $\texttt{Instr}$: Instructions and $\texttt{Ex}$: Examples. See also \autoref{fig:context_mask_graphics}.}}

%\caption{For the prompt contexts of Instructions (\texttt{Instr}) and Examples ($\texttt{Ex}$), $\bullet$: mask, $\circ$: present not masked, $^{-}$: absence. Context highlighted in yellow is masked out from the $j^{\texttt{th}}$ layer onwards. $\texttt{Instr}^{-} \texttt{Ex}^{-}$ is the control condition with no instructions and no examples.}
\label{tab:masking_context_layers_description_wfig}
\end{table*}

==> tables/archive/masking_context_layers_description_wfig.tex <==
 \begin{minipage*}[t]{2.\columnwidth}
  \begin{minipage}[b]{0.25\columnwidth}

    \includegraphics[width=\columnwidth]{images/context_mask_graphics/instr_ex_mask.png}
    %\captionof{}{Schematic of masking context attention for $\texttt{Instr}^{\circ} \texttt{Ex}^{\bullet}.}
    \label{fig:context_masking_fig}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.7\columnwidth}
   \footnotesize
\begin{tabular}{l|c|c|l}

Name  & \texttt{Instr}   & \texttt{Ex}       &  \\
\toprule
% $\texttt{Instr}^{-} \texttt{Ex}^{-}$ & N & N & En: $\cdots$ Fr: \\
% \midrule
\textcolor{blue}{$\overline{\texttt{Ex}}^{Mask}$}  & N & \hl{Y} & \makecell[l]{\hl{En: $\cdots$ Fr: $\cdots$} En: $\cdots$ Fr:} \\
% \midrule
% $\texttt{Instr}^{\bullet}\texttt{Ex}^{-}$ &  \hl{Y} & N & \makecell[l]{\hl{Translate En to Fr:} En: $\cdots$ Fr:} \\

\midrule
%$\texttt{Instr}^{\circ} \texttt{Ex}^{\bullet}$ &  Y  & \hl{Y} & \makecell[l]{Translate En to Fr: \\ \hl{En: $\cdots$ Fr:$\cdots$} En: $\cdots$ Fr:}\\
\textcolor{blue}{$\texttt{Instr},\overline{\texttt{Ex}}^{Mask}$} &  Y  & \hl{Y} & Translate En to Fr: \hl{En: $\cdots$ Fr:$\cdots$} En: $\cdots$ Fr:\\

\midrule
%$\texttt{Instr}^{\bullet} \texttt{Ex}^{\bullet}$ &  \hl{Y} & \hl{Y} & \makecell[l]{\hl{Translate En to Fr:} \\ \hl{En: $\cdots$ Fr:$\cdots$} En: $\cdots$ Fr:} \\
\textcolor{blue}{$\overline{\texttt{Instr}, \texttt{Ex}}^{Mask}$}  &  \hl{Y} & \hl{Y} & \hl{Translate En to Fr:} \hl{En: $\cdots$ Fr:$\cdots$} En: $\cdots$ Fr: \\

\end{tabular}
%\caption{For the prompt contexts of Instructions (\texttt{Instr}) and Examples ($\texttt{Ex}$), $\bullet$: mask, $\circ$: present not masked, $^{-}$: absence. Context highlighted in yellow is masked out from the $j^{\texttt{th}}$ layer onwards. $\texttt{Instr}^{-} \texttt{Ex}^{-}$ is the control condition with no instructions and no examples.}
\label{tab:context_describe}
    \end{minipage}
  \end{minipage*}

==> tables/best_ckpt_L012.tex <==
\begin{table*}[t!]
\begin{tabular}{l|lllll|lllll}

 & Base & No Reg & L0 & L1 & L2 & Base & No Reg & L0 & L1 & L2 \\
 \toprule
  TRAIN \textbackslash TEST & \multicolumn{5}{c}{0-prompts Test (en-fr)} & \multicolumn{5}{c}{5-prompts Test (en-fr)} \\
 \midrule
0-prompts (en-fr) & 18.3 & 21.4 & 20.1 & 20.4 & 20.3 & 24.3 & 24.5 & 24.1 & 21.5 & 21.6 \\
5-prompts (en-fr) & 18.3 & 18.9 & 19.3 & 16.0 & 17.9 & 24.3 & 23.6 & 24.2 & 24.0 & 23.5 \\
% \end{tabular}

% \begin{tabular}{l|lllll|lllll}
\midrule
 & \multicolumn{5}{c}{0-prompts Test (en-pt)} & \multicolumn{5}{c}{5-prompts Test (en-pt)} \\
% \toprule
%  & Base & No Reg & L0 & L1 & L2 & Base & No Reg & L0 & L1 & L2 \\
 \midrule
0-prompts (en-fr) & 6.7 &15.7&8.6&18.6&19.8&25.9 &19.6 &25.8&21.2& 22.6 \\
5-prompts (en-fr) & 6.7 &13.2 &6.4&0.6&10.5 &25.9 &24.3 &26.0&24.5 & 24.1
\end{tabular}
\caption{Filler caption}
\label{tab:best_ckpt}

\end{table*}

==> tables/bloom_layer14_sample.tex <==
\begin{table*}[!t]
\small
\centering
\resizebox{2\columnwidth}{!}{
\begin{tabular}{llrl}
 ID & Generated Translation & Setting & BLEU \\
 \midrule
    62 & Prior to the arrival of troops, Haiti had not encountered problems related to the disease since the 1800s. & 0-prompts w Instr & 2.3 \\
    206 & (None) & 0-prompts w Instr & 0.0 \\
    \midrule
    62  &  Prior to the arrival of troops, Haiti had not encountered problems related to the disease since the 1800s. & 0-prompts w/o Instr & 2.3 \\
    206 &  In France, the first one was made in the city of Paris, in the year of 1968... & 0-prompts w/o Instr & 0.6 \\
    \midrule
    62 & Avant l'arrivée des troupes, Haïti n'avait pas connu de problèmes liés à la fièvre jaune depuis les années 1800. & 5-prompts w Instr & 82 \\
    206 & Dans de nombreuses autres villes d'Italie et dans le reste du monde, en particulier en Pologne.. & 5-prompts w Instr & 67.1 \\ 
    \midrule
    62 & Avant l'arrivée des troupes, Haïti n'avait pas connu de problèmes liés à la fièvre jaune depuis les années 1800. & 5-prompts w/o Instr & 82 \\
    206 & Dans de nombreuses autres villes d'Italie et dans le reste du monde, en particulier en Pologne.. & 5-prompts w/o Instr & 67.1 \\ 
\midrule
ID & Ground Truth Translation & & \\
\midrule
62 & Mais il y a beaucoup de choses sur les oiseaux qui ressemblent encore à un dinosaure. & & \\

206 & Hershey et Chase ont utilisé des phages, ou des virus, pour implanter leur propre ADN.. & & 

\end{tabular}}
\caption{Bloom generated text when masking out layer 14 for different settings, 0 or 5 prompts, and with or without instructions. The test IDs that were selected to be displayed were based on highest variance of BLEU score across layers for the 0-prompt with instruction setting. }
\label{tab:bloom_layer14_sample}
\end{table*}

==> tables/gptneo_layer11_sample.tex <==
\begin{table*}[!t]
%\small
\centering
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{llrl}
 ID & Generated Translation & Setting & BLEU \\
 \midrule
    575 & But there are a lot of things about birds that still look like a dinosaur & 0-prompts w Instr & 2.3 \\
    600 & Hershey and Chase used phages, or viruses, to implant their own DNA into a bacterium & 0-prompts w Instr & 4.8 \\
    \midrule
    575  &  I think it's a good idea to have a little bit of a bird in your pocket. & 0-prompts w/o Instr & 2.6 \\
    600 &  The French have a saying: "The French have a saying: "The French have a saying:.& 0-prompts w/o Instr & 0.0 \\
    \midrule
    575 & Fondamentalement, vous afficherez des annonces pour proposer votre aide, ... & 5-prompts w Instr & 1.3 \\
    600 & Fondamentalement, vous afficherez des annonces pour proposer votre aide,  ... & 5-prompts w Instr & 1.4 \\ 
    \midrule
    575 & Fondamentalement, vous afficherez des annonces pour proposer votre aide, ... & 5-prompts w/o Instr & 1.3 \\
    600 & Fondamentalement, vous afficherez des annonces pour proposer votre aide,  ... & 5-prompts w/o Instr & 1.4 \\
\midrule
ID & Ground Truth Translation & & \\
\midrule
575 & Mais il y a beaucoup de choses sur les oiseaux qui ressemblent encore à un dinosaure. & & \\

600 & Hershey et Chase ont utilisé des phages, ou des virus, pour implanter leur propre ADN.. & & 

\end{tabular}}
%\caption{GPTNeo generated text when masking out layer 11 for different settings, 0 or 5 prompts, and with or without instructions. The test IDs that were selected to be displayed were based on highest variance of BLEU score across layers.}

% \resizebox{\columnwidth}{!}{
% \begin{tabular}{llrl}
%  ID & Generated Translation & Setting & BLEU \\
%  \midrule
%     206 & Prior to the arrival of troops, Haiti had not encountered problems related to the disease since the ... & 0-prompts w Instr & 2.3 \\
%     62 & (None) & 0-prompts w Instr & 0.0 \\
%     \midrule
%     206  &  Prior to the arrival of troops, Haiti had not encountered problems related to the disease since the ... & 0-prompts w/o Instr & 2.3 \\
%     62 &  In France, the first one was made in the city of Paris, in the year of 1968... & 0-prompts w/o Instr & 0.6 \\
%     \midrule
%     206 & Avant l'arrivée des troupes, Haïti n'avait pas connu de problèmes liés à la fièvre jaune depuis les... & 5-prompts w Instr & 82 \\
%     62 & Dans de nombreuses autres villes d'Italie et dans le reste du monde, en particulier en Pologne.. & 5-prompts w Instr & 67.1 \\ 
%     \midrule
%     206 & Avant l'arrivée des troupes, Haïti n'avait pas connu de problèmes liés à la fièvre jaune depuis les ... & 5-prompts w Instr & 82 \\
%     62 & Dans de nombreuses autres villes d'Italie et dans le reste du monde, en particulier en Pologne.. & 5-prompts w Instr & 67.1 \\ 
% \midrule
% ID & Ground Truth Translation & & \\
% \midrule
% 206 & Avant l'arrivée des troupes, Haïti n'avait pas rencontré de problèmes liés à la maladie depuis les... & & \\

% 62 & Dans de nombreuses autres villes d'Italie et dans le reste du monde, en particulier en Pologne, ... & & 

% \end{tabular}}
\caption{Generated text when applying \textit{layer-wise masking} for GPTNeo (layer 11) on \texttt{en}$\rightarrow$\texttt{fr}. We show generated text for 0 or 5 prompts, and with or without instructions. The test IDs that were selected to be displayed were based on highest variance of BLEU score across layers for the 0-prompt with instruction setting. }
\label{tab:bloom_layer14_sample}
\label{tab:gptneo_layer11_sample}

\end{table*}

==> tables/only_gptneo_layer11.tex <==
\begin{table*}[!t]
%\small
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{llrl}
 ID & Generated Translation & Setting & BLEU \\
 \midrule
    575 & But there are a lot of things about birds that still look like a dinosaur & 0-prompts w Instr & 2.3 \\
    600 & Hershey and Chase used phages, or viruses, to implant their own DNA into a bacterium & 0-prompts w Instr & 4.8 \\
    \midrule
    575  &  I think it's a good idea to have a little bit of a bird in your pocket. & 0-prompts w/o Instr & 2.6 \\
    600 &  The French have a saying: "The French have a saying: "The French have a saying:.& 0-prompts w/o Instr & 0.0 \\
    \midrule
    575 & Fondamentalement, vous afficherez des annonces pour proposer votre aide, ... & 5-prompts w Instr & 1.3 \\
    600 & Fondamentalement, vous afficherez des annonces pour proposer votre aide,  ... & 5-prompts w Instr & 1.4 \\ 
    \midrule
    575 & Fondamentalement, vous afficherez des annonces pour proposer votre aide, ... & 5-prompts w/o Instr & 1.3 \\
    600 & Fondamentalement, vous afficherez des annonces pour proposer votre aide,  ... & 5-prompts w/o Instr & 1.4 \\
\midrule
ID & Ground Truth Translation & & \\
\midrule
575 & Mais il y a beaucoup de choses sur les oiseaux qui ressemblent encore à un dinosaure. & & \\

600 & Hershey et Chase ont utilisé des phages, ou des virus, pour implanter leur propre ADN.. & & 

\end{tabular}}
\caption{GPTNeo generated text when masking out layer 11 for different settings, 0 or 5 prompts, and with or without instructions. The test IDs that were selected to be displayed were based on highest variance of BLEU score across layers. More samples of generated text across layers are provided in the Appendix.}
\label{tab:gptneo_layer11_sample}

\end{table*}
